TeV Solar Gamma Rays as a probe for the Solar Internetwork Magnetic Fields

The magnetic fields that emerge from beneath the solar surface and permeate the solar atmosphere are the key drivers of space weather and, thus, understanding them is important to human society. Direct observations, used to measure magnetic fields, can only probe the magnetic fields in the photosphere and above, far from the regions the magnetic fields are being enhanced by the solar dynamo. Solar gamma rays produced by cosmic rays interacting with the solar atmosphere have been detected from GeV to TeV energy range, and revealed that they are significantly affected by solar magnetic fields. However, much of the observations are yet to be explained by a physical model. Using a semi-analytic model, we show that magnetic fields at and below the photosphere with a large horizontal component could explain the $\sim$1 TeV solar gamma rays observed by HAWC. This could allow high-energy solar gamma rays to be a novel probe for magnetic fields below the photosphere.

==> acknowledgements.tex <==


We thank Rasa Muller, Aart Heijboer, and especially Marco Chianese and Suzan Du Pree for useful comments and suggestions. We acknowledge the software packages used, such as the \texttt{SciPy} ecosystem~\cite{scipy} that includes \texttt{Matplotlib} and \texttt{NumPy}; and \texttt{Astropy}~\cite{astropy:2018}. This work was supported by the European Union’s Horizon 2020 research and innovation programme under the Marie Skłodowska-Curie grant agreement No 844664 (KCYN),  JSPS/MEXT KAKENHI Grant Numbers JP17H04836, JP18H04340, JP18H04578 (SA), and the University of Amsterdam (AD and SA).

This project has been carried out in the context of the ``ITFA Workshop'' course, which is part of the joint bachelor programme in Physics and Astronomy of the University of Amsterdam and the Vrije Universiteit Amsterdam, for bachelor students (BB, MG, CG, JG, JH, MJFMJ, LK, WK, SLP, MS, MvH), supervised by KCYN, AD, and SA, following the previous successes~\cite{Aalberts:2018obr, Ando:2019rvr}. The actual work was done in three independent groups A--C during a four-week period of January 2020. Group A (CG, JH, MJFMJ, and WK) worked on the neutrino-flux computation from dark matter decay, and the likelihood analysis. Group B (BB, MG, and LK) worked on the backgrounds and the detector event computation for cascade events. Group C (JG, SLP, MS, and MvH) worked on the backgrounds and the detector event computation for track events. All the group contributed writings and figures for their corresponding sections. 
The entire project was coordinated by the supervisors in group X (KCYN, AD, SA), who collected and checked all the numerical codes developed by the students, added the Monte Carlo simulations, and brought the figures and text to refinement after the course had been completed.



